Perturbative gadgets for gate-based quantum computing: Non-recursive constructions without subspace restrictions

Perturbative gadgets are a tool to encode part of a Hamiltonian, usually the low-energy subspace, into a different Hamiltonian with favorable properties, for instance, reduced locality. Many constructions of perturbative gadgets have been proposed over the years. Still, all of them are restricted in some ways: Either they apply to some specific classes of Hamiltonians, they involve recursion to reduce locality, or they are limited to studying time evolution under the gadget Hamiltonian, e.g., in the context of adiabatic quantum computing, and thus involve subspace restrictions. In this work, we fill the gap by introducing a versatile universal, non-recursive, non-adiabatic perturbative gadget construction without subspace restrictions, that encodes an arbitrary many-body Hamiltonian into the low-energy subspace of a three-body Hamiltonian and is therefore applicable to gate-based quantum computing. Our construction requires $rk$ additional qubits for a $k$-body Hamiltonian comprising $r$ terms. Besides a specific gadget construction, we also provide a recipe for constructing similar gadgets, which can be tailored to different properties, which we discuss.

==> mycommands.tex <==
\usepackage{amsmath}        % For including math equations, theorems, symbols, etc
\usepackage{amssymb}
\usepackage{tikzsymbols}    % for \Cat
\usepackage{dsfont}         % for \mathds
\usepackage{mathrsfs}       % for \mathscr
\usepackage[ruled]{algorithm2e}      % for \begin{algorithm}
% \usepackage{algorithmic}
\usepackage{easy-todo}  % Insert todos with \todo{} 


%----------------------------------------------------------------------------------------
%	OWN COMMANDS
%---------------------------------------------------------------------------------------
\newcommand{\ra}{\rightarrow}
\newcommand{\lra}{\leftrightarrow}
\newcommand{\Ra}{\Rightarrow}
\newcommand{\La}{\Leftarrow}
\newcommand{\LRa}{\Leftrightarrow}
\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}
\newcommand{\II}{\mathds{1}}            %identity

\DeclareMathOperator{\Tr}{Tr}  %trace
\newcommand{\ketbra}[2]{\ket{#1}\!\!\bra{#2}}
% \DeclareMathSymbol{\mathspan}{span}
% \DeclareMathSymbol{\EE}{\mathds{E}}  %expectation
% \DeclareMathSymbol{\argmax}{arg\,max}
% \DeclareMathSymbol{\argmin}{arg\,min}

